Active Crowd Counting with Limited Supervision

To learn a reliable people counter from crowd images, head center annotations are normally required. Annotating head centers is however a laborious and tedious process in dense crowds. In this paper, we present an active learning framework which enables accurate crowd counting with limited supervision: given a small labeling budget, instead of randomly selecting images to annotate, we first introduce an active labeling strategy to annotate the most informative images in the dataset and learn the counting model upon them. The process is repeated such that in every cycle we select the samples that are diverse in crowd density and dissimilar to previous selections. In the last cycle when the labeling budget is met, the large amount of unlabeled data are also utilized: a distribution classifier is introduced to align the labeled data with unlabeled data; furthermore, we propose to mix up the distribution labels and latent representations of data in the network to particularly improve the distribution alignment in-between training samples. We follow the popular density estimation pipeline for crowd counting. Extensive experiments are conducted on standard benchmarks i.e. ShanghaiTech, UCF CC 50, MAll, TRANCOS, and DCC. By annotating limited number of images (e.g. 10% of the dataset), our method reaches levels of performance not far from the state of the art which utilize full annotations of the dataset.

==> tex/sec-method_lyt.tex <==

\begin{figure*}[t]
	\centering
	\includegraphics[width=1\textwidth]{fig/overview3}
	\caption{\small (a) Data taken from SHB (top) and SHA (bottom). (b) B and D stands for the backbone and detection module, respectively; F is the feature map that connects B and D. Anchor boxes (orange) with different scale and aspect ratios are defined on F. Network is trained with both bounding box classification and regression loss, where the regression loss is to compare each box with ground truths within a local band (orange area on F, related to box row $i$).  Ground truth are pseudo ground truth, they are updated iteratively during training based on both box score and size (boxes with green checkmarks are updated). We propose a curriculum learning strategy to feed training samples to the network gradually from easy to hard.
	}
	\label{Fig:intro}
\end{figure*}
\section{Method}\label{Sec:Method}
In this section we first initialize the pseudo ground truth bounding boxes for training; then we present network architecture and pseudo ground truth updating scheme; in the end, we introduce a curriculum learning strategy.

\subsection{Pseudo ground truth initialization}
Supposedly, we have only the ground truth annotations of head centers in training images. To train a detection network, we need to initialize the ground truth bounding boxes for each head. We follow the inspiration in~\cite{zhang2016cvpr} that the head size is indeed related to the distance between the centers of two neighboring heads in crowded scenes. They use it to estimate the Gaussian variance in density map generation. We instead estimate the size  of a bounding-box (the width of a square) $g$ as the center distance $d(g,{\mathrm{NN}_g})$ from $g$ to its nearest neighbor ${\mathrm{NN}_g}$. We call the estimated bounding boxes pseudo ground truth. We show some examples in Fig.~\ref{Fig:intro}(a): the estimations in dense crowds (bottom) are very close to the real ground truth while in sparse crowds (top) are often bigger.

\subsection{Network architecture}
%We follow the famous single stage detector YOLO~\cite{redmon2016cvpr,redmon2017cvpr} that uses features from the entire image to predict each bounding box. The input image is divided into an $S \times S$ grid. If the center of an object falls into a grid cell, that grid cell is responsible for detecting that object.
%We train a specific object class in the network. ResNet-101~\cite{he2016cvpr} is chosen as our backbone. Likewise in ~\cite{hu2017cvpr,najibi2017iccv}, we branch off two streams from the last convolutional layer of the network for both the bounding box classification and regression.
Fig.~\ref{Fig:intro}(b) shows the general architecture of PSDDN. It is a
fully convolutional network which localizes and classifies persons by adding a detection module D on top of feature
map F with stride of 8. The detection module consists
of a convolutional binary classifier and a regressor for detecting
persons and localizing them respectively.

To solve the localization problem, PSDDN follows~\cite{ren2015nips,hu2017cvpr,najibi2017iccv} to regress a set of predefined bounding boxes called anchors to the ground-truth persons. We define the anchors in a dense overlapping sliding window fashion on the feature map F. At each sliding window location, a set of $K$ anchors $A = \{a\}$ are defined which have the same center as that window and different scales and aspect ratios. If F has a size of $W \times H$, there would be $W\times H \times K$ anchors.
%In the implementation details, we will provide the aspect ratio and scale selections in the $M$ anchors.

For the detection module D, a set of convolutional layers
are deployed to extract features for bounding box regression and classification. At each convolution location, the classifier decides whether the windows at the filter center contains a person. A $1 \times 1$ convolutional layer with
$1 \times K$ output channels is used as the classifier. For the regressor branch, another $1 \times 1$ convolutional layer with $4 \times K$
%({?? all or only positive sample for regression})
output channels is deployed. At each location during the
convolution, the regressor predicts the required change in
scale and translation to match each of the positive anchors
to persons.

\subsection{Pseudo ground truth updating}
The pseudo ground truth initialization are not accurate. To train a reliable object detector, we propose to iteratively update the pseudo ground truth in the training images. More formally, let $g^0$ denote a pseudo ground truth bounding box initialized at certain position of an image in epoch $0$. In the network detection module, %where $z$ signifies the down-sampled (by a factor of 8) position on the feature map of the detection module.
positive and negative samples are selected from anchor boxes through their IoU (intersection-over-union) with $g^0$. Over the positive samples, we choose the one with the highest classification score; if its width or height (we judge on the smaller one to allow some occlusion among objects) is smaller than $d(g, {\mathrm{NN_g}})$,
%from head $g$ to its nearest head ${\mathrm{NN}_{g}}$,
it will replace the pseudo ground truth $g^0$ in next epoch. We denote by $g^1$ the corresponding ground truth at epoch 1. All the pseudo ground truth bounding boxes will be updated iteratively after every epoch as long as the condition satisfies.

The proposed updating scheme is similar to the typical two-step learning scheme in weakly supervised object detection (WSOL)~\cite{song2014icml,shi2016eccv,papadopoulos2016cvpr,cinbis2017pami}. In a typical WSOL setting, people do not know the object locations in the training images but only the image-level object class labels. They alternates the learning process between (a) re-training the object detector given the current selection of instances, and (b) re-localizing object instances in the images using the current object detector.
The process separates model training and inference explicitly.
While in PSDDN, the re-localizing step is integrated within model training. Since we know the accurate head centers in a image, this guarantees that the bounding box at every head point is updated, and it is much faster than explicit inference.
Recalling that our bounding box initialization are bigger than or close to the real ground truth,
it provides us a good starting point for model convergence.
%In a typical WSOL setting, we do not know the object locations in the training images but only the image-level object class labels. The training process starts by training the object detector using complete images as training samples.
\subsection{Bounding box regression}
We first refer to~\cite{girshick2014cvpr} for some notations in  bounding box regression. The anchor bounding box $a = (ax, ay, aw, ah)$ specifies the pixel coordinates of the center of the bounding box together with $a$'s width and height in pixels. $a$'s corresponding ground truth $g$ is specified in the same way: $g = (gx, gy, gw, gh)$. %We drop the subscript position index for now.
We parameterize the transformation required from $a$ to $g$ as four variables $d_x(a)$,  $d_y(a)$,  $d_w(a)$,  $d_h(a)$. The first two specify a scale-invariant translation of the center of $a$, while the second two specify log-space translations of the width and height of $a$. These variable are produced from bounding box regressor; we can use them to transform $a$ into a predicted ground-truth bounding box $\hat g = (\widehat{gx}, \widehat{gy}, \widehat{gw}, \widehat{gh})$:
\begin{equation}\label{Eq:boundingbox}
 \begin{aligned}
\widehat{gx} = {aw} \cdot d_x(a) + ax,~
\widehat{gy} &= {ah}\cdot d_y(a) + ay\\
\widehat{gw} = {aw}\cdot \mathrm{exp}({d_w(a)}),~
\widehat{gh} &= {ah}\cdot \mathrm{exp}({d_h(a)})\\
 \end{aligned}
\end{equation}
The target is therefore to minimize the difference between $g$ and $\hat g$.

The ground truth $g$ in our framework is a pseudo ground truth: the center coordinates $gx$, $gy$ are accurate but the width and height $gw$, $gh$ are not. Based on this, we can first define a loss function $l_{xy}$ regarding the center distance between $g$ and $\hat g$:
\begin{equation}\label{Eq:Lregxy}
%lxy = (gx - \widehat{gx})^2 + (gy - \widehat{gy})^2.
lxy = (\frac{gx-ax}{aw} -  \frac{\widehat{gx}-ax}{aw})^2 + (\frac{gy-ay}{ah} - \frac{\widehat{gy}-ay}{ah})^2.
\end{equation}
With respect to the loss function on width and height, it is not realistic to directly compare between $g$ and $\hat g$. We instead build upon the observation that in a crowd image bounding boxes of persons along the same horizontal line should have similar size.
%while \textbf{ii)} boxes along the vertical line should have decreased size in general from the near front to the far end of the image.
This is inspired from the perspective map widely used in the crowd counting task~\cite{chan2008cvpr,zhang2015cvpr,huang2018tip}: its values are increased from the top to the bottom; and are equal in the same row. Two assumptions are made to generate the perspective map: first, there is no in-plane rotation; second, the ground in the captured scene is flat. In standard crowd counting benchmarks, both assumptions holds for most of the images. Hence, we propose to penalize the predicted bounding boxes $\hat g$ if its width and height clearly violate the above observation.

More formally, we denote $ g_{ij} = \{{gx}_{ij}, {gy}_{ij},{gw}_{ij},{gh}_{ij})$ as the pseudo ground truth bounding at position $ij$ on the feature map. We notice that $i$ and $j$ are in fact equivalent to ${gx}$ and ${gy}$, we keep both for our convenience. We first compute the mean and standard deviation of the width (heights) of bounding boxes within a narrow band area (row: $i-1: i+1$; column: $1:W$) on the feature map (\eg orange band on F in Fig.~\ref{Fig:intro}(b)). We use $G_i$ to denote the set of ground truth head positions within the narrow band related to $i$. The corresponding statistics are:
\begin{equation}\label{Eq:Lregsigma}
\begin{aligned}
 \mu w_{i} &= \frac{1}{|G_i|}\sum_{{mn} \in G_i}{gw}_{mn}\\
 \sigma w_i&=\sqrt{\frac{1}{|G_i|}\sum_{{mn} \in G_i}({gw}_{mn} - \mu {w}_i)^2},\\
% \overline{gh}_{i} &= \frac{1}{3H}\sum_{k=i-1}^{i+1}\sum_{j=1}^H\widehat{gh}_{kj},\\
% \sigma(\widehat{gh}_i)&=\sqrt{\frac{1}{3H}\sum_{k=i-1}^{i+1}\sum_{j=1}^H(\widehat{gh}_{kj} - \overline{gh}_i)^2}\\
 \end{aligned}
\end{equation}
where $|G_i|$ denote the the cardinality of the set. $\mu {h}_{i}$ and $\sigma{h}_i$ can be obtained in the same way. We adopt a three-sigma rule that if the predicted bounding box width $\widehat{gw}_{ij}$ is larger than $\mu w_{i} + 3\sigma w_i$ or smaller than $\mu w_{i} - 3\sigma w_i$ we will penalize it; otherwise not. The loss function $lw_{ij}$ regarding the width of bounding box $\hat g_{ij}$ is thus defined as:
\begin{equation}\label{Eq:Lregwh}
%lw_{ij} = \begin{cases} (\widehat{gw}_{ij} - (\mu w_{i} + 3\sigma w_i))^2 & \widehat{gw}_{ij} > \mu w_{i} + 3\sigma w_i \\ ((\mu w_{i} - 3\sigma %w_i) - \widehat{gw}_{ij})^2 & \widehat{gw}_{ij} < \mu w_{i} - 3\sigma{w_i} \\0 & otherwise \end{cases}
lw_{ij} = \begin{cases} (\ln{\frac{\widehat{gw}_{ij}}{aw}} - \ln{\frac{(\mu w_{i} + 3\sigma w_i)}{aw}})^2 & \widehat{gw}_{ij} > \mu w_{i} + 3\sigma w_i \\ (\ln{\frac{(\mu w_{i} - 3\sigma w_i)}{aw}} - \ln{\frac{\widehat{gw}_{ij}}{aw}})^2 & \widehat{gw}_{ij} < \mu w_{i} - 3\sigma{w_i} \\0 & otherwise \end{cases}
\end{equation}
Similarly, we can obtain $lh_{ij}$. We do not require a restrict compliance with \textbf{i} and \textbf{ii} in a local area. Instead we design the narrow band and three-sigma rule for the tolerance of head size variation among individuals.

The overall bounding box regression loss $L\mathrm{reg}$ for one image is given by:
\begin{equation}\label{Eq:Lreg}
L\mathrm{reg} = \sum_{ij \in G } lxy_{ij} + lw_{ij} + lh_{ij},
\end{equation}
where $G$ to denote the set of ground truth head points in one image.

%Similarly, we can obtain the corresponding statistics at line $i+1$: $\overline{gw}_{i+1}$, $\sigma(\widehat{gw}_{i+1})$, $\overline{gh}_{i+1}$, $\sigma(\widehat{gh}_{i+1})$; as well as line $i-1$: $\overline{gw}_{i-1}$, $\sigma(\widehat{gw}_{i-1})$, $\overline{gh}_{i-1}$, $\sigma(\widehat{gh}_{i-1})$.

\subsection{Curriculum learning}
Conventional training scheme learns a model on the entire training set at the same time. However, generalizing on either very sparse or very dense crowds can be very difficult in our point-supervised setting. The former is due to the inaccuracy of the bounding box initialization, which can be much bigger than the size of real ground truth in sparse crowds; while the latter is limited by the discriminative ability of the deep network. Both cases are likely to corrupt the model and result in bad detections. To avoid it, we introduce a curriculum learning strategy to learn the model gradually from easy to hard.

The difficulty of training images is related to both the crowd density and pseudo ground truth accuracy. We propose to split the training set $\mathcal I$ into $Z$ ($Z$ = 3) folds according to their crowd densities. We denote by $\mathcal I_1$, $\mathcal I_2$, $\mathcal I_3$ the corresponding fold with samples of crowd density \emph{medium}, \emph{very sparse} and \emph{very dense}, respectively.   We start by running PSDDN on the first fold $\mathcal I_1$, containing images of medium crowd density with accurate initial ground truth. Training on this fold will lead to a reasonable detection model $\mathcal A_1$. We run PSDDN on $\mathcal I_1$ for a couple of epochs to get a solid $\mathcal A_1$. The process then moves on to the second fold $\mathcal I_2$, which contains very sparse crowds, adding all its images into the current working set $\mathcal I_1 \cup \mathcal  I_2$ and running PSDDN again. Instead of starting from scratch, we use $\mathcal A_1$ to update the pseudo ground truth in $\mathcal I_2$ such that the updated bounding boxes are tighter on persons. The model $\mathcal A_2$ output by PSDDN on $\mathcal I_1 \cup \mathcal  I_2$ is fine-tuned from $\mathcal A_1$ and will be better than it, as it is trained from more samples. The detection of persons in $\mathcal I_1$ will also improve. The process will iteratively move on to batch $\mathcal I_3$ and run PSDDN on the joint set $\mathcal I_1 \cup \mathcal  I_2 \cup \mathcal  I_3$. By the time the process reaches batch $\mathcal  I_3$ with small and heavily occluded persons, the model will already be very good and will do a much better job than training all the samples together from the very beginning. Note that we empirically choose Z = 3 as it works best.
%The proposed curriculum learning strategy enables the model generalization of PSDDN from very sparse crowds to very dense crowds.
%On one hand, the algorithm works better on samples of sparse crowds, which have few occlusion between individuals; on the other hand, the algorithm works better on samples of dense crowds
%
%\begin{table}[htbp]
%	\caption{\label{tab:test}示例表格}
%	\begin{tabular}{c}
%		\toprule
%		Point-supervised deep detection network\\
%		\midrule
%	    \textbf{Initialization:}\\
%	    1) split the training set $\mathcal I$ into 3 folds \\
%		2) initialize pseudo ground truth bounding boxes in fold $\mathcal I_1$ \\
%		3) train an appearance model $\mathcal A_1$ on $\mathcal I_1$\\
%		for fold k = 1:3 do \\
%		\bottomrule
%	\end{tabular}
%\end{table}

%We present our overall algorithm in xx.
\medskip
The network is trained with a multi-task loss for both classification and bounding box regression. The classification loss is the same with~\cite{girshick2015iccv,ren2015nips} while the regression loss is defined in~(\ref{Eq:Lreg}). We follow a same online hard mining scheme with~\cite{hu2017cvpr}.


